Medically Aware GPT-3 as a Data Generator for Medical Dialogue Summarization

In medical dialogue summarization, summaries must be coherent and must capture all the medically relevant information in the dialogue. However, learning effective models for summarization require large amounts of labeled data which is especially hard to obtain. We present an algorithm to create synthetic training data with an explicit focus on capturing medically relevant information. We utilize GPT-3 as the backbone of our algorithm and scale 210 human labeled examples to yield results comparable to using 6400 human labeled examples (~30x) leveraging low-shot learning and an ensemble method. In detailed experiments, we show that this approach produces high quality training data that can further be combined with human labeled data to get summaries that are strongly preferable to those produced by models trained on human data alone both in terms of medical accuracy and coherency.

==> sections/exp_old.tex <==

\section{Experiments and Results}

\noindent \textbf{Model terminology}
We introduce the following shorthands to aid the discussion
\begin{itemize}
    \item \textbf{\gptthree}: GPT-3 few-shot priming approach adapted to the medical snippet summarization task (\autoref{sec:gpt3})
    \item \textbf{\gptthreecf}: GPT-3 few-shot priming approach adapted to the medical snippet summarization task, ensembled using concept forcing  (\autoref{sec:gpt3cf})
    \item \textbf{\pegasus}: Abstractive summarization model \cite{zhang2019pegasus}
    \item \textbf{\twompgen}: Pretrained pointer-generator model with generator loss introduced in \cite{joshi2020dr}, referred therein as 2M-PGEN
\end{itemize}

\noindent \textbf{Implementation Details}: We used GPT-3 via the API released by OpenAI\footnote{\url{https://beta.openai.com/}}. Maximum response length was set to 128 tokens, temperature was set to 0.6, while the presence and frequency penalties were both set to 0. \TODO{Maybe in the appendix we can give an example of how we prompt GPT-3 to produce a summary. Not sure if this would be that useful in the paper itself. We can add if we have space, however.}

We borrowed most parameter settings for \twompgen from \cite{joshi2020dr} for fine-tuning it on the CNN-Dailymail dataset. It was then fine-tuned on our summarization task dataset with a batch size of 16, source\_max\_tokens = 400, response\_max\_tokens = 200 and max\_grad\_norm clipped at 2.0, for two epochs with a learning rate of 0.15 using Adagrad optimizer. We used a beam size of 4 for decoding.

We used the \pegasus implementation that is fine-tuned on CNN-Dailymail\footnote{\url{https://huggingface.co/google/pegasus-cnn_dailymail}} provided by \cite{wolf-etal-2020-transformers}. We fine-tuned it on our summarization task dataset with an effective batch size of 256, source\_max\_tokens = 512, response\_max\_tokens = 128 for two epochs with a learning rate of \TODO{fill} using Adafactor optimizer. We again used a beam size of 4 for decoding.

\subsection{Main Results: Efficacy of \textbf{\gptthreecf}}
\label{subsec:cf-help}

{\it Human-Doctor Evaluation:} perform doctor evaluation on these results shown in

\autoref{fig:gpt3cf_human_eval} which validate that the ensembled approach captures relevant medical information and more often produces better summaries overall.


\autoref{tab:gpt3-cf} provides our main results comparing GPT-3 with our proposed approach (\textbf{\gptthreecf}: Algorithm~\autoref{alg:gpt3-cf}). We make the following observations:
\begin{itemize}
    \item Proposed approach shows lift across all automated metrics, even when we ensembled with two times the data (comparison between $H_{21}$ and $H_{42}$
    \item As we increase the number of  ensembling trials, $K=\{2,3,5,10\}$ (and corresponding datasets $ H_{42},H_{63}, H_{105}$ and $H_{210}$),  \textbf{\gptthreecf}  shows improvements in terms of capture relevant medical information ( Negation and Concept F1 scores) and also more closely overlapping with ground truth summary, as measured by ROUGE score
\end{itemize}
%We consider $K=\{2,3,5,10\}$ number of ensembling trials. From , we observe that (1) The ensembling approach lifts all automated metrics and (2) automated metrics increase as $K$ increases. 


Due to computational limits and metric saturation we don't experiment with larger values of $K$ and enable ensembling with $K=10$ trials in all further experiments.

\begin{table}[ht!]
\renewcommand{\arraystretch}{1.2}
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{c|c|c|c|c}
\hline
\multirow{2}{*}{\textbf{Models}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Train Data}\\\textbf{Source}\end{tabular}} & \multicolumn{3}{c}{\textbf{Metrics}} \\
\cline{3-5}
 & & \begin{tabular}[c]{@{}c@{}}\textbf{Negation}\\\textbf{F1}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Concept}\\\textbf{F1}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{ROUGE-L}\\\textbf{F1}\end{tabular} \\
\hline
\gptthree & $H_{21} $ & 44.96 & 56.98 & 56.55 \\
\hline
\multirow{4}{*}{\gptthreecf} & $H_{42}$ & 46.58 & 60.45 & 58.70 \\
& $H_{63}$ & 47.72 & 61.42 & 58.24 \\
& $H_{105}$ & 48.78 & 62.27 & 58.59 \\
& $H_{210}$ & \textbf{50.16} & \textbf{63.01} & \textbf{59.05} \\

\hline
\end{tabular}
\end{adjustbox}
\caption{Automated evaluation of GPT-3-based summarization approaches.}
\label{tab:gpt3-cf}
\end{table}

\begin{figure}
\begin{adjustbox}{width=\columnwidth}
    \centering
    \includegraphics{figures/gpt3_en_human_eval.png}
\end{adjustbox}
\caption{Doctor evaluation of amount of medical information covered by summaries provided by \gptthree vs \gptthreecf approaches and which ones they considered ``best''}
\label{fig:gpt3cf_human_eval}
\end{figure}

\subsection{Can GPT-3 simulated data be used to train summarization models?}
\label{subsec:sim-train}
We now evaluate the efficacy of the idea introduced in \autoref{subsec:gpt3-data-sim} of using GPT-3 as a data simulator. We compare \pegasus and \twompgen trained on human labeled data H$_{6400}$ and GPT-3 synthesized data using ensembling GCF$^{K=10}_{6400}$. Note that synthesizing GCF$^{K=10}_{6400}$ needed all of 21$\times$10$=$210 human labeled examples. In essence, \emph{210 labeled examples + ensembling using GPT-3 are able to yield comparable performance to a model trained on 6400$(\sim$30x) human labeled examples.} \TODO{maybe discuss amenability of data to pegasus vs drsum?}. The performance gain between \twompgen trained on GPT-3 labeled data vs Dr. summarize trained on human labeled data is much larger than the performance gain between Pegasuss trained on GPT-3 labeled data vs Dr. Summarize labeled data. We conclude that this is due to the fact that Dr. Summarize is a hybrid abstractive-extractive summarization model. Our human labelers were instructed to copy as much as possible from the source when synthesizing a summary to encourage Dr. Summarize to generate words less often than it would copy. GPT-3 does not have this instruction when synthesizing summaries and hence we conclude that this is the reason for the performance difference. \TODO{First pass on this; pretty terrible description need to clean up language}

\begin{table}[ht!]
\renewcommand{\arraystretch}{1.2}
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{c|c|c|c|c}
\hline
\multirow{2}{*}{\textbf{Models}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Train Data}\\\textbf{Source}\end{tabular}} & \multicolumn{3}{c}{\textbf{Metrics}} \\
\cline{3-5}
 & & \begin{tabular}[c]{@{}c@{}}\textbf{Negation}\\\textbf{F1}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Concept}\\\textbf{F1}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{ROUGE-L}\\\textbf{F1}\end{tabular} \\
\hline
\multirow{4}{*}{\pegasus} & $H_{6400}$ & 21.09 & 35.96 & 55.59 \\
& $GCF_{6400}^{k=10}$ & 28.89 & 40.02 & 53.43 \\
& $GCF_{12800}^{k=10}$ & 26.70 & 40.21 & 56.66 \\
& $GCF_{25600}^{k=10}$ & 28.61 & 40.58 & 58.44 \\
$\alpha=0.5$ & \begin{tabular}[c]{@{}c@{}} $H_{6400} + GCF_{3200}^{k=10}$ \end{tabular} & \textbf{30.14} & \textbf{43.49} & \textbf{62.45} \\
$\alpha=1$ & \begin{tabular}[c]{@{}c@{}} $H_{6400} + GCF_{6400}^{k=10}$\end{tabular} & 30.70 & 43.73 & 60.63 \\
$\alpha=2$ & \begin{tabular}[c]{@{}c@{}} $H_{6400} + GCF_{12800}^{k=10}$\end{tabular} & 29.43 & 41.02 & 59.85 \\
$\alpha=3$ & \begin{tabular}[c]{@{}c@{}} $H_{6400} + GCF_{25600}^{k=10}$\end{tabular} & 31.93 & 44.68 & 61.05 \\
\hline
\multirow{4}{*}{\twompgen} &$H_{6400}$ & 26.75 & 39.95 & 52.70 \\
& GCF_{6400}^{k=10} & 24.29 & 37.55 & 48.47 \\
& GCF_{12800}^{k=10} & 26.66 & 38.49 & 49.18 \\
& GCF_{25600}^{k=10} & 26.08 & 39.47 & 50.85 \\
$\alpha=0.5$ & \begin{tabular}[c]{@{}c@{}}$H_{6400} + GCF_{3200}^{k=10}$\end{tabular} & \textbf{27.51} & \textbf{40.46} & \textbf{53.39} \\
$\alpha=1$ & \begin{tabular}[c]{@{}c@{}}$H_{6400} + GCF_{6400}^{k=10}$\end{tabular} & 27.18 & 40.36 & 40.46 \\
$\alpha=2$ & \begin{tabular}[c]{@{}c@{}}$H_{6400} + GCF_{12800}^{k=10}$\end{tabular} & 27.9 & 40.68 & 53.07 \\
$\alpha=3$ & \begin{tabular}[c]{@{}c@{}}$H_{6400} + GCF_{25600}^{k=10}$\end{tabular} & 26.33 & 39.89 & 53.07 \\

\hline
\end{tabular}
\end{adjustbox}
\caption{Automated evaluation of summarization models trained with different data labeling methodology \TODO{the dataset names need to be refined}}
\label{tab:results}
\end{table}

\subsection{Does more and more GPT-3 synthesized data yield better performance?}
\label{subsec:more-train}
To test this hypothesis we create $GCF_{12800}^{k=10}$ and  $GCF_{12800}^{k=10}$ and again train both \pegasus and \twompgen on these datasets. As shown in \autoref{tab:results}, we observe that more GPT-3 synthesized data does not seem to help too much in terms of Concept and Negation F1's and saturate. The Rouge-L F1, seems to improve steadily. This aligns with our qualitative analysis indicating that more and more data leads to better coherency of the summaries; however the ability to retain medical information does not seem to increase.  \TODO{why?}

\subsection{How do models trained on a mix of human and GPT-3 synthesized data compare to those trained on either?}
\label{subsec:mix-train}

To evaluate this, we experimented with $\alpha=0.5, 1, 2, 3$ where $\alpha$ is the fraction of the amount of human labeled data from GPT-3 we mix. For instance, with 6400 human labeled examples, $\alpha=0.5$ implies the dataset contains 6400 human labeled examples along with $0.5*6400=3200$ GPT-3 synthesized examples.

As shown in \autoref{tab:results}, we observe that $\alpha=0.5$ yields the best performance across different $\alpha$ values. We also observe that for both architectures \pegasus and \twompgen, model trained on mixed training data is much better than those trained on only GPT-3 synthesized data or only human labeled data. \TODO{I anticipate questions around why we did not try weighting here. Our experiments suggest that when human data is weighed more than gpt-3 we get better performance. Could this be true for higher amounts of GPT-3 data with more weight on human data?} 

\TODO{Jai: Good point, showing all our  mix data its not entirely clear that higher weights is better for human data is it? Especially since we are operating on one run and the metrics at different alphas are so close. What did we get evalutated by the humans for the mix? Did we get anything evaluated?}

% \subsection{Results}

% {\noindent \bf Improvements as a summarizer. }
% Main results results with and without concept forcing

% {\noindent \bf Importance of "K"}
% Results as a function of “k” summaries/ shots

% {\noindent \bf As a data labeler}
%  GPT-3 as the training data for existing models


\begin{figure}
\begin{adjustbox}{width=\columnwidth}
    \centering
    \includegraphics{figures/pegasus_human_eval.png}
\end{adjustbox}
\caption{Doctor evaluation of amount of medical information covered by summaries provided by \pegasus models and which ones they considered ``best''}
\label{fig:pegasus_human_eval}
\end{figure}

\begin{figure}
\begin{adjustbox}{width=\columnwidth}
    \centering
    \includegraphics{figures/drsum_human_eval.png}
\end{adjustbox}
\caption{Doctor evaluation of amount of medical information covered by summaries provided by \twompgen models and which ones they considered ``best''}
\label{fig:pegasus_human_eval}
\end{figure}

% \begin{table}[ht!]
% \renewcommand{\arraystretch}{1.2}
% \begin{adjustbox}{width=\columnwidth}
% \begin{tabular}{c|c|c|c|c|c}
% \hline
% \multirow{2}{*}{\textbf{Models}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Data}\\\textbf{Source}\end{tabular}} & \multicolumn{4}{c}{\textbf{Human eval}} \\
% \cline{3-6}
%  & & All & Most & Some & None \\
% \hline
% \multirow{2}{*}{\pegasus} & H-6.4k & 227 & 93 & 93 & 88
% & G-6.4k & 257 & 87 & 72 & 85 \\
% $\alpha=0.5$ & H-6.4k+G-3.2k & 296 & 86 & 55 & 64 \\
% \hline
% \multirow{2}{*}{\twompgen} & H-6.4k & 21.09 & 35.96 & 55.59 \\
% & G-6.4k & 28.89 & 40.02 & 53.43 \\
% $\alpha=0.5$ & H-6.4k+G-3.2k & \textbf{30.14} & \textbf{43.49} & \textbf{62.45} \\

% \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Automated evaluation of summarization models trained with different data labeling methodology \TODO{the dataset names need to be refined}}
% \label{tab:results}
% \end{table}

==> sections/model.tex <==
\section{Approach}

Labeled data, especially in a specialized domain such as medicine, is hard to obtain. This section describes how GPT-3, a large pre-trained language model, can be leveraged in a few-shot learning setting for the task of medical dialogue summarization. We discuss two approaches- 
\begin{enumerate}
    \item Using GPT-3 directly as a summarizer
    \item Using GPT-3 as a source of noisy labels to train summarization models 
\end{enumerate}

\textbf{GPT -3}: In 2020, OpenAI developed GPT-3, a neural language model that is capable of sophisticated natural language generation and completion of tasks like classification, question-answering, and summarization. While OpenAI has not open-sourced the model’s code or pre-trained weights at the time of writing, it has built an API to experiment with the model’s capacity. In order to generate subject-specific text, GPT-3 requires nothing more than a few short prompts that are representative
of the text one wants the model to emulate.

\subsection{GPT-3 as a summarizer}

As in \TODO{cite GPT-3}, we \emph{prime} GPT-3 by providing it a task description, a prompt of $N$ labeled examples. Note that $N$ is upper-bounded by the maximum context window length of GPT-3. We then use this primed GPT-3 to label unlabeled data as shown in Algorithm~\ref{gpt3}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}
  \caption{GPT-3 summarizer}
  \label{gpt3}
  \begin{algorithmic}[1]
    \Require{dialogue text $T$, set $S$ containing $N$ labeled examples, GPT3} 
    \Ensure{summary of $T$}
    \State $\texttt{summary} \gets \texttt{GPT3}(S, T)$
  \State \Return $\texttt{summary}$
  \end{algorithmic}
\end{algorithm}

\subsubsection{Medical concept forcing}
A medical dialogue summarizer must capture medical concepts and findings that were discussed in the dialogue to be effective. Since GPT-3 is not specifically trained on the medical domain, it does not always succeed in doing so.

A simple approach to address this called concept forcing is presented as Algorithm~\ref{gpt3_cf}. In this approach, we use the GPT3 summarizer $L$ times using $L$ different seed sets of labeled examples and choose the summary that captures the most number of medical concepts in the source text. This approach assumes access to a medical concept extractor that identifies the medical concepts in a given piece of source text. \TODO{can refer to UMLS and point out that approach is independent of the choice of extractor}. \TODO{should we add why this approach is simplistic and provide examples of when we might not want to capture all concepts?}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}
  \caption{GPT-3 summarizer with concept forcing}
  \label{gpt3_cf}
  \begin{algorithmic}[1]
    \Require{dialogue text $T$, medical concept extractor $E$, max\_tries $L$, universe $U$ of labeled examples, GPT3} 
    \Ensure{summary of $T$ that preserves maximum number of medical concepts in $T$}
      \State $\texttt{best} \gets \texttt{null}$
      \State $C \gets E(T)$
      \State $\texttt{num\_found} \gets 0$
      \For{$i \gets 1, \cdots, L$} 
        \State $S \gets \text{sample $N$ examples from $U$}$
        \State $\texttt{summary} \gets \texttt{GPT3}(S, T)$
        \State $C_s \gets E(\texttt{summary})$
        \State $I \gets C \cap C_s$
        \If {$\vert I \vert = \vert C \vert$}
            \State \Return $\texttt{summary}$
        \ElsIf {$\vert I \vert > \texttt{num\_found}$}
            \State $\texttt{num\_found} \gets |I|$
            \State $\texttt{best} \gets \texttt{summary}$
        \EndIf
      \EndFor
      \State \Return $\texttt{best}$
  \end{algorithmic}
\end{algorithm}

\subsection{GPT-3 as data source}
An alternative to using GPT-3 summaries as the final summaries is to use GPT-3 to label an unlabeled set of examples and use these ``noisily labeled" examples to train a separate summarization model. There are several reasons why this approach might be preferred. To list a few,
\TODO{needs work, expand}
\begin{enumerate}
    \item HIPAA
    \item control over model architecture
    \item external dependency
\end{enumerate}


==> sections/model_1.tex <==
\section{Background: GPT-3 {\it as} medical conversation summarizer}
\label{sec:gpt3}

GPT-3 \cite{brown2020language} is a pre-trained language model that can be applied in few-shot setting.  In particular, at inference time, the  model is primed with a text description of the task and a few demonstrations of the task (with no gradient updates to the model) to perform the same task on a previously unseen example. For our task of medical conversation summarization,  this translates to providing a few example pairs of (source text, target text) as input context, and then have the model predict the target text for a new source text. \TODO{See Appendix for an example prompt}

Following this paradigm, we \emph{prime} GPT-3 by providing it a prompt of $N$ (typically N=21, as upper-bounded by the maximum context window length) manually labeled snippet-summary pairs. Table~\ref{tab:examples} provides examples of summarization obtained by using this technique. As we can see, while the summaries are linguistically correct, GPT-3, on its own,  suffers from a number of problems. First, it misses a number of important pieces of information in the snippets -- missing any medical concepts can often make the summary unusable (See row 1--3). Second, the model may not always get the affirmations correct (See row 4). Thirdly, the summary itself may not be coherent (see row 5)

\input{sections/examples}
\section{Our approach: Medically-aware GPT-3 summarizer}
\label{sec:gpt3cf}
Our approach to using GPT-3 as a medical conversation summarizer hinges on two key insights:
First, as GPT-3 is a few shot learner, we found that the model can be sensitive to the priming context provided. While one approach to solve this may be to provide GPT-3 with  most informative context for a task, this is daunting task on its own, and can potentially  be tackled if we had large number of labeled examples (which is the exact problem we want to tackle with GPT-3). Drawing on the learnings from vast literature in ensembling techniques \TODO{cite}, our first key insight is that if we can generate multiple summaries from GPT-3 given a variety of contexts, then we should be able to ensemble these outputs to identify the summary that is consistent with the dialog input. 
    
Unlike a classification task where the output is a fixed label space, it is not clear how one can ensemble textual summaries. Hence our second key insight is to not ensemble multiple summaries for the same input, but identify the best one based on the important requirement of the task. Since we care about the correctness of the medical concepts being captured, we need a ensembling function that identifies the best summary that has the captured the most medical information in the dialog input. For this purpose, we use an in house medical entity recognizer, which we describe next. 

Algorithm~\ref{alg:gpt3-cf} provides an overview of our approach to medically aware GPT-3 ensemble {\textbf{\gptthreecf}}. We assume access a small set of labeled examples $\mathcal{L}$. For each input dialog text, $D$, we get $K$ summaries, by invoking GPT-3 each time with $N$ examples sampled randomly from $\mathcal{L}$. We also assume access to a  medical entity extractor that can discern the medical concepts from both the source text and the algorithm returns the best summary that covers the most accuracy in terms of capturing the medical concepts in the source text


\begin{algorithm}
  \caption{Medically aware GPT-3 ensemble summarizer (\textbf{\gptthreecf}) }
  \label{alg:gpt3-cf}
  \begin{algorithmic}[1]
    \Require{dialogue snippet $T$,  ensembling trials $K$, universe $\mathcal{L}$ of labeled examples, medical entity extractor $MedicalEntityRecognizer$, GPT3} 
   % \Ensure {Best summary for $T$ that preserves medical information in $T$ }
      \State $C^* \gets MedicalEntityRecognizer(T)$
      \For{$i \gets 1, \cdots, K$} 
        \State $S \gets \text{sample $N$ examples from $L$}$
        \State $\texttt{summary}_i \gets \texttt{GPT3}(S, T)$
        \State $C_i \gets MedicalEntityRecognizer(\texttt{summary}_i)$
      \EndFor
       \State $best \gets \argmax_{i} \frac{|C_i \cap C^*|}{|C_i \cup C^*|} $
        \State \Return $\texttt{summary}_{best}$
  \end{algorithmic}
\end{algorithm}

\noindent{\textsc{MedicalEntityRecognizer}:} We use an in-house medical concept extractor that identifies the medical concepts from a given piece of source text. The \textsc{MedicalEntityRecognizer} method takes piece of text (dialogue or a summary) as the input and returns a set of medical concepts present in the text. Internal to this method is access to universe of medical concepts based on Unified Medical Knowledge Systems \footnote{\url{https://www.nlm.nih.gov/research/umls/index.html}}. Note that any medical entity recognizer can be used \TODO{cite} that has coverage for all medical concepts such as patient symptoms, disorders, laboratory tests and medications that are common in these medical conversations. 


\subsection{Our proposed model as a data generator}
We extend the above approach to view GPT-3 as a labeled data generator. In particular, we use our approach to collect a large amount of labeled examples that serves as inputs to training an off-the-shelf summarization model. This view tackles the problem of using GPT-3 in a real world application where the patient's conversation (in its raw form) needs to be exchanged with an external third party such as OpenAI/GPT-3 which may not have design/privacy regulations around HIPAA. However, with the help of experts, its easy to ensure that the snippets that will be part of the training set is chosen to follow privacy laws.
\label{subsec:gpt3-data-sim}


==> sections/model_2.tex <==
\newcommand{\myindent}[1]{\newline\makebox[#1cm]{}}

\section{GPT-3 as Data Generator}
\label{sec:gpt3cf}
We are interested in a model that uses only a small amount of human labeled data to learn an effective medical dialogue summarizer. At the same time, we want such a model to be used in the practical setting where patient privacy can be protected, and the privacy agreement between the patient and the providing service is respected.


In order to achieve these two goals, we propose a medically aware ensemble, \textbf{\gptthreecf}, that uses GPT-3 \cite{brown2020language} language model within an inner loop, and is effective at medical summarization. We then leverage this model as a data generator to obtain a large training set \footnote{Unlike data at inference time, training data is fixed and can be ensured to be privacy protected} to train an in-house medical dialogue summarization model. Such an in-house model can be used at inference time without the practical constraints related to protecting patient privacy that would require full de-identification to be applied in any conversation, if we were to access the GPT-3 service.



%The need for these models as data simulator arise from the practical constraints related to protecting patient privacy that would require full de-identification to be applied to any conversation before accessing the GPT-3 service. 


\subsection{Can GPT-3 serve as a  medical summarizer?}
To be able to generate a training set for a medical summarization task, we first need to verify if GPT-3 is a good summarizer. GPT-3 takes as input a {\it priming context} to perform the task on a previously unseen example. Priming context refers to the text description of a task and a few demonstrations for the task. 
% \TODO{See Appendix for an example prompt for our task of medical summarization}. 

Table~\ref{tab:examples} column 2 provides examples of summaries when we used the GPT-3 API. Clearly, we can see that it misses a number of important pieces of information in the snippets -- first, missing medical concepts making the summary unusable (Rows 1-2). Second, the model may not always get the affirmations correct (Row 3). Third, the summary may repeat redundant information from the doctor's queries (Row 4).

While this may lead to {\it misconceiving} GPT-3 as ineffective for summarization task, we show next that by ensembling and infusing medical knowledge, GPT-3 can be used as part of an effective low-shot learning approach to medical summarization.

%For our task of medical conversation summarization,  this translates to providing a few example pairs of (source text, target text) as input context, and then have the model predict the target text for a new source text. 
\input{sections/examples}

\subsection{\gptthreecf: Medically-aware ensemble of GPT-3}
Our biggest learning in exploring GPT-3 is that it is sensitive to the priming context provided as the model does not learn but just adheres to the examples given. While one approach may be to provide GPT-3 with the most informative context for a task, this itself is a daunting task and can potentially be tackled if we had a large number of labeled examples (which is the exact problem we want to tackle with GPT-3).

Drawing on the learning from vast literature in ensembling techniques \cite{bishop1995neural}, our first key insight is that if we can generate multiple summaries from GPT-3 using a variety of priming contexts, then we should be able to ensemble these outputs to identify the summary that is ideal for the dialogue. This insight leads to a question on how to ensemble multiple text summaries. The answer to this question relies in the core requirement for medical summarization: We care about the coverage of medical concepts mentioned and therefore the best ensembling function is the one that returns the summary with the most medical information in the dialog input. 

In Algorithm~\ref{alg:gpt3-cf} we provide our approach to the medically aware GPT-3 ensemble {\textbf{\gptthreecf}}. We assume access to a small set of labeled examples $\mathcal{L}$. For each input dialog snippet, $D$, we get $K$ summaries, by invoking GPT-3 each time with $N$ examples sampled randomly without replacement from $\mathcal{L}$. We also assume access to a medical entity extractor that can discern the medical concepts from both the dialogue snippet and the summary. The algorithm returns the best summary that has the highest recall in terms of capturing the medical concepts in the dialogue. For this purpose, we use an in-house medical concept extractor \textsc{MedicalEntityRecognizer} that can identify medical concepts from a given piece of text. This extractor has access to the universe of medical concepts based on Unified Medical Knowledge Systems \footnote{\url{https://www.nlm.nih.gov/research/umls/index.html}}, which includes patient symptoms, disorders, laboratory tests and medications. Note that any medical entity recognizer ({\it cf.} \cite{concept19} and references therein) that has coverage for all these types of medical concepts found in medical conversations can be used.
\begin{algorithm}
  \caption{Medically aware GPT-3 ensemble summarizer (\textbf{\gptthreecf}) }
  \label{alg:gpt3-cf}
  \begin{algorithmic}[1]
    \Require{dialogue snippet $T$,  ensembling trials $K$, universe $\mathcal{L}$ of labeled examples, medical entity extractor $MedicalEntityRecognizer$, GPT3} 
   % \Ensure {Best summary for $T$ that preserves medical information in $T$ }
      \State $C^* \gets MedicalEntityRecognizer(T)$
      \For{$i \gets 1, \cdots, K$} 
        \State $S \gets \text{sample $N$ examples from $L$}$
        \State $\texttt{summary}_i \gets \texttt{GPT3}(S, T)$
        \State $C_i \gets MedicalEntityRecognizer( \myindent{1.1} \texttt{summary}_i)$
      \EndFor
       \State $best \gets \argmax_{i} \frac{|C_i \cap C^*|}{|C^*|} $
        \State \Return $\texttt{summary}_{best}$
  \end{algorithmic}
\end{algorithm}

Reconsider Table~\ref{tab:examples} for qualitative comparison between \gptthree and \gptthreecf.  We can see that summaries obtained using \gptthreecf capture the medical concepts comprehensively (shown in bold) and also have better grammatical structure. We also quantitatively validate the summaries on a small data set distinct from what is used for priming(see \S ~\ref{sec:doceval} for guidelines). In \autoref{fig:gpt3_best}, based on doctor evaluation, we can see that \gptthreecf is significantly better at summarization than \gptthree.
\begin{figure}[ht!]
    \centering
    \includegraphics[scale=0.5]{figures/gpt3_best.png}
\caption{Doctor evaluation of which among \gptthree and \gptthreecf summaries they considered ``best'' showing that \gptthreecf is a better approach for labeling}
\label{fig:gpt3_best}
\end{figure}



\subsection{\gptthreecf as a data labeler}
Based on the qualitative and quantitative results above, we use \gptthreecf as our 
labeled data generator. In particular, we use our approach to collect a large amount of labeled examples that serves as inputs to training an off-the-shelf summarization model. This view tackles the problem of using GPT-3 in a real world application where the patient's conversation (in its raw form) needs to be exchanged with an external third party such as OpenAI/GPT-3 which may not have design/privacy regulations around HIPAA. However, with the help of experts, it's easy to ensure that the dialogues that will be part of the training set are chosen following privacy protocols.
\label{subsec:gpt3-data-sim}



%Following this paradigm, we \emph{prime} GPT-3 by providing it a prompt of $N$ (typically N=21, as upper-bounded by the maximum context window length) manually labeled snippet-summary pairs. 

==> sections/qual_old.tex <==
\begin{table}[]
\tiny
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{p{0.14\textwidth}p{0.14\textwidth}p{0.14\textwidth}}
\hline
\textbf{Snippet} & \textbf{GPT-3} & \textbf{GPT-3 with concept forcing} \\
\hline
\begin{tabular}[c]{@{}p{0.14\textwidth}@{}}
\textbf{DR}: Thanks for answering my questions. Apart from the benadryl and hydrocortisone have you used any thing to help? \\ \textbf{PT}: No, that's everything
\end{tabular} & Hasn't used any thing to help & Used nothing else to help other than Benadryl and hydrocortisone. \\
\hline
\begin{tabular}[c]{@{}p{0.14\textwidth}@{}}
\textbf{DR}: I see. How long did the episode last back then? Have you noticed similar symptoms previously as well? \\ \textbf{PT}: But its not severe to the point as right \\ \textbf{PT}: 10-15 minutes \\ \textbf{PT}: I dont do excersie \\ \textbf{PT}: But my heart rate goes a little higher when i did excerice long time ago
\end{tabular} & Episode lasted 10-15 minutes. Did not notice similar symptoms previously. Heart rate goes a little higher during exercise. & It lasted 10-15 minutes. She doesnt do excersie. Her heart rate goes a little higher when she did excerice long time ago. \\
\hline
\begin{tabular}[c]{@{}p{0.14\textwidth}@{}}
\textbf{DR}: Oh, and at what age was she diaper-trained in the first place? \\ \textbf{PT}: It was at age 3 \\ \textbf{PT}: 2 1/2- 3.I can't really remember
\end{tabular} & It was at age 3. & She was diaper trained at age 3. 2 1/2-3. Can't remember. \\
\hline
\begin{tabular}[c]{@{}p{0.14\textwidth}@{}}
\textbf{DR}: Do you have pain when you notice penile discharge? \\ \textbf{PT}: no i'm not
\end{tabular} & Did not notice penile discharge. No pain. &  Doesn't have pain when noticing penile discharge. \\
\hline
\begin{tabular}[c]{@{}p{0.14\textwidth}@{}}
\textbf{DR}: I have a few questions to ask. How long have you been having this vaginal discomfort? \\ \textbf{PT}: only a few days, since like friday or saturday maybe
\end{tabular} & I have a few questions to ask. How long has she been having vaginal discomfort? & Has been having vaginal discomfort for only a few days, since friday or saturday. \\
\hline
\begin{tabular}[c]{@{}p{0.14\textwidth}@{}}
\textbf{DR}: Thank you so much for sharing. Are you on any regular medications for that? \\ \textbf{PT}: My only regular medication is birth control -Apri. Low dosage.
\end{tabular} & On birth control. & Only regular medication is birth control -Apri. Low dosage. \\
\hline
\begin{tabular}[c]{@{}p{0.14\textwidth}@{}}
\textbf{DR}: You had mentioned the headache starting after stopping the medications. Have you had similar headache while stopping medications before? \\ \textbf{PT}: Yes \\ \textbf{PT}: Well that's a complicated question \\ \textbf{PT}: I'm not really sure \\ \textbf{DR}: Okay, no worries. Wanted to know a bit more since you had mentioned about them. That's all.
\end{tabular} & Yes. Stopping medications before. &  Yes, has headache while stopping medications before. Is not sure. \\
\hline
\end{tabular}
\caption{Snippets along with summaries produced by GPT-3, without and with concept forcing \TODO{Pick the most salient 3-4 examples}}
\label{tab:examples}
\end{table}

